Task Agnostic and Post-hoc Unseen Distribution Detection

Despite the recent advances in out-of-distribution(OOD) detection, anomaly detection, and uncertainty estimation tasks, there do not exist a task-agnostic and post-hoc approach. To address this limitation, we design a novel clustering-based ensembling method, called Task Agnostic and Post-hoc Unseen Distribution Detection (TAPUDD) that utilizes the features extracted from the model trained on a specific task. Explicitly, it comprises of TAP-Mahalanobis, which clusters the training datasets' features and determines the minimum Mahalanobis distance of the test sample from all clusters. Further, we propose the Ensembling module that aggregates the computation of iterative TAP-Mahalanobis for a different number of clusters to provide reliable and efficient cluster computation. Through extensive experiments on synthetic and real-world datasets, we observe that our approach can detect unseen samples effectively across diverse tasks and performs better or on-par with the existing baselines. To this end, we eliminate the necessity of determining the optimal value of the number of clusters and demonstrate that our method is more viable for large-scale classification tasks.

==> WACV 2023_ Task-Agnostic OOD Detection_arxiv/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> WACV 2023_ Task-Agnostic OOD Detection_arxiv/wacv/main_paper/sections/00_abstract.tex <==
Despite the recent advances in out-of-distribution(OOD) detection, anomaly detection, and uncertainty estimation tasks, there do not exist a task-agnostic and post-hoc approach.
To address this limitation, we design a novel clustering-based ensembling method, called {\bf T}ask {\bf A}gnostic and {\bf P}ost-hoc {\bf U}nseen {\bf D}istribution {\bf D}etection (TAPUDD) that utilizes the features extracted from the model trained on a specific task. Explicitly, it comprises of \emph{TAP-Mahalanobis}, which clusters the training datasets' features and determines the minimum Mahalanobis distance of the test sample from all clusters. Further, we propose the \emph{Ensembling module} that aggregates the computation of iterative \emph{TAP-Mahalanobis} for a different number of clusters to provide reliable and efficient cluster computation.
Through extensive experiments on synthetic and real-world datasets, we observe that our \edit{task-agnostic} approach can detect unseen samples effectively across diverse tasks and performs better or on-par with the existing \edit{task-specific} baselines. 
We also demonstrate that our method is more viable \edit{even} for large-scale classification tasks.

==> WACV 2023_ Task-Agnostic OOD Detection_arxiv/wacv/main_paper/sections/01_introduction.tex <==
\section{Introduction}

Deep neural networks have achieved phenomenal performance in diverse domains such as computer vision and healthcare~\cite{bojarski2016end,mikolov2013efficient,dermato16deep}. However, they struggle to handle samples from an unseen distribution, leading to unreliable predictions and fatal errors in safety-critical applications.
In an ideal situation, a robust model should be capable of making predictions on samples from the learned distributions, and at the same time, flag unknown inputs from unfamiliar distributions so that humans can make a responsible decision. 
For instance, in safety-critical tasks such
as cancer detection, the machine learning assistant must issue a warning and hand over the control to the doctors when it detects an unusual sample that it has never seen during training. Thus, in practice, it is important for a  model to know when \textit{not} to predict. This task of detecting samples from an unseen distribution is referred to as out-of-distribution (OOD) detection~\cite{hendrycks2017base,liang2017enhancing,mahala18,sastry2021gram,liu2020energy,Huang2021MOSTS,Hendrycks2019ABF,sehwag2021ssd,Xiao2021DoWR,mahmood2020multiscale}.


Most of these OOD detection methods mainly focusing on classification tasks have shown great success. However, they are not directly applicable to other tasks like regression.
Although a few bayesian and non-bayesian techniques ~\cite{gal2016dropout,lakshminarayanan2017simple,maddox_2019_simple,Graves2011PracticalVI} estimate uncertainty in regression tasks, they are not post-hoc as it often requires a modification to the training pipeline, or multiple trained copies of the model, or training a model with an optimal dropout rate.
This raises an under-explored question:
\begin{quote}
\vspace{-1.2mm}
\textit{Can we design a task-agnostic, and
post-hoc approach for unseen distribution detection 
% across diverse tasks
?}
\vspace{-1.2mm}
\end{quote}


Motivated by this, we propose a novel clustering-based ensembling framework, \quotes{{\bf T}ask {\bf A}gnostic and {\bf P}ost-hoc {\bf U}nseen {\bf D}istribution {\bf D}etection (TAPUDD)}, which comprises of two modules, \emph{TAP-Mahalanobis} and \emph{Ensembling}. \emph{TAP-Mahalanobis} partitions the training datasets' features into clusters and then determines the minimum Mahalanobis distance of a test sample from all the clusters. 
The \emph{Ensembling }module aggregates the outputs obtained from \emph{TAP-Mahalanobis} iteratively for a different number of clusters. It enhances reliability and eliminates the need to determine an optimal number of clusters. \edit{
Since TAPUDD is a post-hoc approach and doesn't require training the model, it is more efficient and easy to deploy in real-world.
}

To demonstrate the efficacy of our approach, we conduct experiments on 2-D synthetic datasets for binary and multi-class classification tasks and observe that our method effectively detects the outliers in both tasks. Further, we extensively evaluate our approach on real-world datasets for diverse tasks. In particular, we evaluate our approach for binary classification (gender prediction) and regression (age prediction) task on RSNA boneage dataset to detect the samples shifted by brightness. We observe that our method successfully identifies the shifted samples. We also evaluate our approach on large-scale classification tasks and obtained logical performance on diverse OOD datasets. To sum up, our contributions include:
\begin{itemize}
\setlength{\itemsep}{1.5pt}
\setlength{\parskip}{0pt}
\setlength{\parsep}{0pt}

\item We propose a novel task-agnostic and post-hoc approach, \textbf{TAPUDD}, to detect unseen samples across diverse tasks like classification, regression, etc. 
\item For the first time, we empirically show that a single approach can be used for multiple tasks with stable performance. 
We conduct exhaustive experiments on synthetic and real-world datasets for regression, binary classification, and multi-class classification tasks to demonstrate the effectiveness of our method.
\item \edit{We conduct ablation studies to illustrate the effect of number of clusters in \emph{TAP-Mahalanobis} and ensembling strategies in TAPUDD. We observe that TAPUDD
performs better or on-par with \emph{TAP-Mahalanobis} 
and eliminates the necessity to determine the optimal number of clusters.}
\end{itemize} 

==> WACV 2023_ Task-Agnostic OOD Detection_arxiv/wacv/main_paper/sections/02_related_work.tex <==
\section{Related Work}
\label{sec:related_work}
To enhance the reliability of deep neural networks, there exist several efforts along the following research directions:

\parahead{Out-of-distribution Detection}
Recent works have introduced reconstruction-error based~\cite{Schlegl2017UnsupervisedAD,Zong2018DeepAG,Deecke2018ImageAD,Pidhorskyi2018GenerativePN,Perera2019OCGANON,Choi2020NoveltyDV}, density-based~\cite{ren2019likelihood,choi2018waic,mahmood2020multiscale,Du2019ImplicitGA,Grathwohl2020YourCI,Nalisnick2019DetectingOI,Serr2020InputCA}, and self-supervised~\cite{Golan2018DeepAD,Hendrycks2019UsingSL,Bergman2020ClassificationBasedAD,sehwag2021ssd} OOD detection methods. Other efforts
include post-hoc methods~\cite{mahala18,liu2020energy,hendrycks2017base,liang2017enhancing,sastry2021gram,Hendrycks2019ABF,Nalisnick2019DoDG} that do not require modification to the training procedure. 
However, there is no approach that is post-hoc and does not require the class label information of the training data.

\parahead{Uncertainty Estimation} 
Research in this direction primarily estimates the uncertainty to enhance the robustness of networks in regression tasks.
Well-known methods to estimate uncertainty include bayesian~\cite{Mackay1992BayesianMF,Neal1995BayesianLF,Blundell2015WeightUI,Graves2011PracticalVI,Louizos2016StructuredAE,Hasenclever2017DistributedBL,Li2015StochasticEP,korattikara2015bayesian,Welling2011BayesianLV,Springenberg2016BayesianOW,maddox_2019_simple} and non-bayesian~\cite{gal2016dropout,lakshminarayanan2017simple} approaches, which have shown remarkable success.
However, they require significant modification to the training pipeline, multiple trained copies of the model, and are not post-hoc.


\parahead{Anomaly Detection} 
This task aims to detect anomalous samples shifted from the defined normality. Prior work~\cite{Perera2019OCGANON,Wang2019EffectiveEU,Golan2018DeepAD,Schlegl2017UnsupervisedAD,Chalapathy2018AnomalyDU,Zong2018DeepAG,Deecke2018ImageAD} proposed methods
to solve anomaly detection.
However, more recently, ~\cite{sehwag2021ssd,Tack2020CSIND,Bergman2020ClassificationBasedAD,HernndezLobato2015ProbabilisticBF} proposed a unified method to solve both OOD detection and anomaly detection. Nonetheless, these methods require end-to-end training and are not post-hoc.

There exist no unified approach to enhance the reliability of neural networks across distinct tasks like classification, regression, etc.
In contrast to all the aforementioned efforts, our work presents a post-hoc, and task-agnostic approach to detect unknown samples across varied tasks.

==> WACV 2023_ Task-Agnostic OOD Detection_arxiv/wacv/main_paper/sections/03_background_method.tex <==
\section{Background and Methodology}
\label{sec:background_method}
% We first provide the problem formulation and the essential background. Then, we propose our task-agnostic and post-hoc approach for unseen distribution detection.

\subsection{Problem Formulation} 
\label{sec:problem_formulation}
We assume that the in-distribution data $\mathcal{D}_{\text{IN}} =\{ X, Y \}$ is composed of $N$ i.i.d. data points with inputs $X=\{\mathbf{x}_1, ..., \mathbf{x}_N\}$ and labels $Y=\{y_1, ..., y_N\}$.
Specifically, $\mathbf{x}_i\in \mathbb{R}^{d}$ represents a $d$-dimensional input vector, and $y_i$ is its corresponding label. For classification problems, the label $y_i$ is one of the $C$ classes.
For regression problems, the label is real-valued, that is $y_i\in \mathbb{R}$. For autoencoding (or self-supervised or unsupervised learning tasks), the label $y_i$ is absent.
Let $f : X \rightarrow \mathcal{Z}$, where $\mathcal{Z}\in \mathbb{R}^{m}$,  denote the feature extractor often parameterized by a deep neural network which maps a sample
from the $d$-dimensional input space \edit{($X$)} to the $m$-dimensional feature space ($\mathcal{Z}$). 

Our goal is to obtain the feature of a sample from a trained DNN
using the feature extractor ($f$), and equip it with an OOD detector which can detect samples from different distribution than the training distribution (OOD samples) or samples shifted from the training distribution based on some attribute
\cite{Park2021NaturalAS}. We wish to design a task-agnostic, and post-hoc OOD detector which only requires the features of training data obtained from the trained model. Since such OOD detector does not require the raw training data, it minimizes privacy risk, a significant advantage for tasks where data-related privacy is a serious concern.

\subsection{Background}

\parahead{Mahalanobis distance-based OOD detection method} Mahalanobis OOD detector~\cite{mahala18} approximates each class as multi-variate gaussian distribution and use the minimum Mahalanobis distance of a test sample from all classes for OOD detection. \editr{Given that density estimation in high-dimensional space is a known intractable problem, Mahalanobis approach is viewed as a reasonable approximation that has been widely adopted.}
In particular, it fits the gaussian distribution to the features of the  training  data $X=\{(\mathbf{x}_1, y_1), \ldots, (\mathbf{x}_N, y_N)\}$ and compute per-class mean 
\resizebox{.4\hsize}{!}{ $\mathcal{\mu}_{c} = \frac{1}{N_{c}} \sum_{i:y_{i}=c}^{} f(\mathbf{x}_{i})$ } and a shared covariance matrix 
\resizebox{.8\hsize}{!}{ $\Sigma = \frac{1}{N} \sum_{c=1}^{C} \sum_{i:y_{i}=c}^{} (f(\mathbf{x}_{i}) - \mathcal{\mu}_{c}) (f(\mathbf{x}_{i}) - \mathcal{\mu}_{c})^{T},$ }
where $f(\mathbf{x}_{i})$ 
denotes the penultimate layer features of an input sample $\mathbf{x}_i$, $C$ denotes the total number of classes in the training dataset, and $N_c$ denotes the total number of samples with class label $c$.
Given a test sample $\mathbf{x}_{test}$, the mahalanobis score is defined as:
% 
\vspace{-0.8mm}
\begin{equation}
\resizebox{0.95\hsize}{!}{
$\mathcal{S}_{\text{Mahalanobis}} = -\min\limits_{c} (f(\mathbf{x}_{test}) - \mathcal{\mu}_{c})^{T} \Sigma ^{-1}(f(\mathbf{x}_{test}) - \mathcal{\mu}_{c}),$
\nonumber
}
\vspace{-0.8mm}
\end{equation}
where $f(\mathbf{x}_{test})$ denotes the penultimate layer features of a test sample $\mathbf{x}_{test}$.

\begin{figure*}[t]
\centering
    \vspace{-2mm}
     \includegraphics[width=0.9\textwidth]{wacv/main_paper/figures/TAPUDD.pdf}
     \vspace{-1mm}
     \caption{
    \edit{\textbf{TAPUDD.} Our method first extracts the features of an input image $\mathbf{x}$ from the feature extractor $f$ of a model trained on a specific task. \emph{TAP-Mahalanobis} module then uses the extracted features $f(\mathbf{x}_{train})$ to fit the gaussian mixture model and computes the minimum mahalanobis distance $S_k$ for the given feature vector $f(\mathbf{x}_{test})$.
    Further, the \emph{Ensembling} module aggregates the mahalanobis distance ($S_{k1}$ to $S_{kn}$) obtained from iterative computation of \emph{TAP-Mahalanobis} for different number of clusters ($k_1$ to $k_n$)
    to enhance the reliability.
    } 
     }
    %  \vspace{-1mm}
     \label{fig:method}
\end{figure*}

% \vspace{4mm}
\subsection{TAPUDD: {\bf T}ask {\bf A}gnostic and {\bf P}ost-hoc {\bf U}nseen {\bf D}istribution {\bf D}etection}
\label{sec:tapudd}

We propose a novel, {\bf T}ask {\bf A}gnostic and {\bf P}ost-hoc {\bf U}nseen {\bf D}istribution {\bf D}etection (TAPUDD)  method, as shown in \cref{fig:method}. The method comprises of two main modules \emph{TAP-Mahalanobis} and \emph{Ensembling}.\\

% \vspace{-2pt}
\parahead{TAP-Mahalanobis} Given training samples $X=\{\mathbf{x}_1, ..., \mathbf{x}_N\}$, we extract the features of the in-distribution data from a model trained for a specific task using a feature extractor $f$. We then pass these features to the \emph{TAP-Mahalanobis} module. It first partition the features of the in-distribution data into $K$ clusters using Gaussian Mixture Model (GMM) with \quotes{\textit{full}} covariance. Then, we model the  features in each cluster independently as multivariate gaussian and compute the empirical cluster mean and covariance of training samples $X=\{\mathbf{x}_1, ..., \mathbf{x}_N\}$ 
and their corresponding cluster labels $C=\{c_1, ..., c_N\}$ as:
\vspace{-0.8mm}
\begin{equation}
\resizebox{.98\hsize}{!}{
    % \small
    $\mathcal{\mu}_{c} = \frac{1}{N_{c}} \sum_{i:c_{i}=c}^{}f(\mathbf{x}_{i}),
    \Sigma_{c} = \frac{1}{N_{c}} \sum_{i:c_{i}=c}^{} (f(\mathbf{x}_{i}) - \mathcal{\mu}_{c}) (f(\mathbf{x}_{i}) - \mathcal{\mu}_{c})^{T},$
    \nonumber
    }
\vspace{-0.8mm}
\end{equation}
where $f(\mathbf{x}_{i})$ denotes the penultimate layer features of an input sample $\mathbf{x}_i$ from a cluster $c_i$.

Then, given a test sample, $\mathbf{x}_{test}$, we obtain the negative of the minimum of the Mahalanobis distance from the center of the clusters as follows:
\vspace{-0.8mm}
\begin{equation}
\resizebox{.97\hsize}{!}{
    $\mathcal{S}_{\text{TAP-Mahalanobis}} = -\min \limits_{c} (f(\mathbf{x}_{test}) - \mathcal{\mu}_{c})^{T} \Sigma_{c} ^{-1} (f(\mathbf{x}_{test}) - \mathcal{\mu}_{c}),$
    \nonumber
    }
\vspace{-0.8mm}
\end{equation}
where $f(\mathbf{x}_{test})$ denotes the penultimate layer features of a test sample $\mathbf{x}_{test}$.
We then use the score $\mathcal{S}_{\text{TAP-Mahalanobis}}$ to distinguish between ID and OOD samples. To align with the conventional notion of having high score for ID samples and low score for OOD samples, negative sign is applied.

However, it is not straightforward to determine the value of the number of clusters $K$ for which the OOD detection performance of \emph{TAP-Mahalanobis} is optimal for different tasks and datasets. To illustrate the effect of using a different number of clusters $K$ in \emph{TAP-Mahalanobis} on the OOD detection performance, we conduct an ablation in \cref{sec:ablations}.
To this end, we present an \emph{Ensembling} module.\\

\begin{figure*}
\centering
% \fbox{%
\vspace{-2mm}
\begin{minipage}[t]{0.4\linewidth}
    \centering
    \includegraphics[width=0.75\linewidth]{wacv/main_paper/figures/experiments/synthetic_data_TAPMOS_vs_TAP-UDD_round.pdf}
    \caption{ID score landscape of TAP-MOS and TAPUDD on synthetic 2-D binary and multi-class classification datasets.
    A sample is \edit{deemed} as OOD when it has a
    % % low ID score(\textcolor{blue}{blue color}).
    \textcolor{blue}{\textbf{low ID score}}.
    The \textbf{\textcolor{magenta}{Pink Points}} represent the in-distribution data; \textbf{\textcolor{red}{Red Triangles}} and \textbf{\textcolor{orange}{Orange Diamonds}} represent the far and near OOD samples, respectively. 
    \edit{TAP-MOS fails to detect certain OOD samples, whereas TAPUDD effectively detects all OOD samples.}
    }
    \label{fig:synthetic_data_UMOS}
\end{minipage}%
% }
\hfill
% \fbox{%
\begin{minipage}[t]{0.58\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{wacv/main_paper/figures/experiments/synthetic_data_multi-class_TAPmahala_vs_TAPUDD_round.pdf}
    \caption{ID score landscape of \emph{TAP-Mahalanobis} for different values of $K$ (\ie , number of clusters); and TAPUDD for different ensemble variations on synthetic 2D multi-class classification dataset. A sample is deemed as OOD when it has a \textcolor{blue}{\textbf{low ID score}}. The \textbf{\textcolor{magenta}{Pink Points}} represent the in-distribution data.
    Results demonstrate that \emph{TAP-Mahalanobis} does not perform well for some values of $K$ whereas TAPUDD with all ensembling strategies perform better or on-par with \emph{TAP-Mahalanobis}. 
    }
    \label{fig:synthetic_data_umahala_vs_tauood}
\end{minipage}
% }
% \vspace{-3mm}
\vspace{-1mm}
\end{figure*}

\vspace{-3mm}
\parahead{Ensembling} This module not only eliminates the need to determine the optimal value of $K$ but also provides more reliable results. \edit{We obtain \emph{TAP-Mahalanobis} scores for different values of $K \in [k_{1}, k_{2}, k_{3}, ..., k_{n}]$ and aggregate them to obtain an ensembled score, $\mathcal{S}_{\text{Ensemble}}$. This ensures that a sample is detected as OOD only if a majority of the participants in ensembling agrees with each other. }

% \editr{Note that Mahalanobis distance (MD) is an optimal choice only if the training distribution follows the Gaussian distribution.
% However, we believe that MD in TAPUDD is safe since the \emph{Ensembling} module does a \textit{reasonably simple approximation} by aggregating the MD obtained from GMM with a different number of clusters. Please refer to Sec. \appendixsecs{4} of the Appendix for a detailed discussion.}

\parahead{Remark} \editr{We empirically compare GMM with K-means and observe that GMM is more flexible in learning the cluster shape in contrast to K-means, which learned spherical cluster shapes. Consequently, K-means performs poorly when detecting OOD samples near the cluster.
Other popular clustering methods such as agglomerative clustering or DBSCAN are less compatible with Mahalanobis distance and require careful hyperparameter adjustment, such as the linking strategies for agglomerative clustering or the epsilon value for DBSCAN. 
Please refer to \cref{sec:discussion} for a detailed discussion on GMM clustering.
}

% \vspace{-1mm}
\subsection{Ensembling Strategies}
\edit{Given the dependency of TAPUDD on the aggregation of \emph{TAP-Mahalanobis} scores obtained for different values of $K$ (\ie , number of clusters)}
, a natural question arises: \textit{how do different ensembling strategies affect the performance of unseen distribution detection}? To answer this, we systematically consider the following five ensembling strategies:

\vspace{2pt}
\parahead{Average} We consider $\mathcal{S}_{\text{TAP-Mahalanobis}}$ obtained from \emph{TAP-Mahalanobis} module for different $K$ with equal importance and average them to obtain an 
ensembled score, $\mathcal{S}_{\text{Ensemble}}$.

\vspace{2pt}
\parahead{Trimmed Average} For certain values of $K$, the \emph{TAP-Mahalanobis} module can provide extremely high or extremely low $\mathcal{S}_{\text{TAP-Mahalanobis}}$. Therefore, to reduce bias caused by extreme \emph{TAP-Mahalanobis} scores, we eliminate \quotes{$m$} \emph{TAP-Mahalanobis} scores from top and bottom and then take the average of the remaining $n_e > K/2$ \emph{TAP-Mahalanobis} scores to obtain a final ensembled score.  

\vspace{2pt}
\parahead{Seesaw} In general, the voting ensemble in regression tasks includes the average of all participants. However, some participants might completely disagree with the other participants, and including all of them in ensembling might provide inaccurate results. 
To this end, we present \quotes{\textit{seesaw}} ensembling strategy wherein we sort the \emph{TAP-Mahalanobis} scores obtained for different values of $K$ and average the $n_e > K/2$ participants that agree with each other.
In other words, if a majority of participants agree to a high \emph{TAP-Mahalanobis} score, we pick the top $n_e$ participants; otherwise, we select the bottom $n_e$ participants. 

\vspace{2pt}
\parahead{Top} 
\edit{We sort the \emph{TAP-Mahalanobis} scores obtained for different values of $K$ and then obtain the ensembled score $\mathcal{S}_{\text{Ensemble}}$ by averaging the top $n_e > K/2$ scores.}

\vspace{2pt}
\parahead{Bottom}  
\edit{We sort the \emph{TAP-Mahalanobis} scores obtained for different values of $K$ and average the bottom $n_e > K/2$ scores to obtain an ensembled score $\mathcal{S}_{\text{Ensemble}}$.}

==> WACV 2023_ Task-Agnostic OOD Detection_arxiv/wacv/main_paper/sections/04_experiments.tex <==
\section{Experiments and Results}
In this section, we validate our approach, TAPUDD, by conducting experiments on 2-D synthetic datasets 
(\cref{sec:synthetic_dataset_experiments}). To further bolster the effectiveness of our method, we present empirical evidence to validate TAPUDD on several real-world tasks, including binary classification  (\cref{sec:binary_classification_experiments}), regression (\cref{sec:regression_experiments}), and 
\edit{large-scale}
classification (\cref{sec:multi_classification_experiments}).  For binary classification and regression task, we evaluate our approach on Natural Attribute-based Shift (NAS) detection dataset. In NAS detection, a sample is shifted from the training distribution based on attributes like brightness, age, etc. Throughout all experiments, we use TAP-MOS, a task-agnostic and post-hoc extension of MOS\cite{Huang2021MOSTS}, as an additional baseline. Unlike the original MOS where class hierarchy was used to do clustering, we perform GMM clustering. 
\edit{More details on TAP-MOS are provided in \cref{sec:supp_tapmos}.}

\input{wacv/main_paper/tables/binary_class_nas_detection}


\subsection{Evaluation on Synthetic Datasets}
\label{sec:synthetic_dataset_experiments}

\parahead{Experimental Details} We generate synthetic datasets 
in $\mathbb{R}^{2}$ for binary classification and multi-class classification tasks. The in-distribution (ID) data $\mathbf{x}\in \mathcal{X} = \mathbb{R}^{2}$ is sampled from a Gaussian mixture model (refer to \cref{sec:supp_synthetic_data_gen} for more details). All the samples except the ID samples in the 2-D plane represent the OOD samples. We consider the 2-D sample as the penultimate layer features on which we can directly apply OOD detection methods like TAPUDD, \emph{TAP-Mahalanobis}, and TAP-MOS. 

\vspace{2pt}
\parahead{TAPUDD outperforms TAP-MOS}
We compare the OOD detection performance of TAP-MOS and TAPUDD. ~\cref{fig:synthetic_data_UMOS}\textcolor{red}{a} and ~\cref{fig:synthetic_data_UMOS}\textcolor{red}{b} presents the ID score landscape of TAP-MOS and TAPUDD for binary classification and multi-class classification, respectively. The \textbf{\textcolor{magenta}{Pink Points}} represent the in-distribution data; \textbf{\textcolor{red}{Red Triangles}} and \textbf{\textcolor{orange}{Orange Diamonds}} represent far and near OOD samples, respectively. Here for TAP-MOS, we present results using number of clusters as $2$ and $8$ in binary classification and multi-class classification, respectively. 
For TAPUDD, we present the results of the \quotes{\textit{average}} ensembling strategy computed across the number of clusters in $[1, 2, 3, 4, 5, 6, 7, 8, 9, 10, 16, 32]$.
We observe that our proposed approach TAPUDD detects all OOD samples effectively. We also notice that TAP-MOS fails to detect OOD samples
near or far from the periphery of all the clusters
% (\textbf{\textcolor{red}{Red Triangles}} and \textbf{\textcolor{orange}{Orange Diamonds}} in binary classification; \textbf{\textcolor{red}{Red Triangles}} in multi-class classification)
.
Thus, to understand the scenarios where TAPMOS fails to identify OOD, we conduct a detailed analysis of the MOS approach in \cref{sec:supp_analysis} and observe that it also fails for the similar corner cases. 

% \vspace{1pt}
\parahead{TAPUDD outperforms TAP-Mahalanobis}
We  present a comparison to demonstrate the effectiveness of TAPUDD against \emph{TAP-Mahalanobis} in \cref{fig:synthetic_data_umahala_vs_tauood}. 
We present the ID score landscape of \emph{TAP-Mahalanobis} for different values of $K$ and TAPUDD with different ensemble variations for multi-class classification in a 2-D synthetic dataset.
The \textbf{\textcolor{magenta}{Pink Points}} represent the in-distribution data. We observe that for certain values of $K$, \emph{TAP-Mahalanobis} fails to detect some OOD samples. However, all ensemble variations in TAPUDD effectively detect OOD samples and performs better, or on par, with \emph{TAP-Mahalanobis}. 
Thus, TAPUDD eliminates the necessity of choosing the optimal value of $K$.
We also provide results on a 2-D synthetic dataset for binary classification in \cref{sec:supp_additional_exp}.

\input{wacv/main_paper/tables/regression}

\subsection{NAS Detection in Binary Classification}
\label{sec:binary_classification_experiments}

\parahead{Experimental Details}
\edit{We use the RSNA Bone Age dataset~\cite{013a4b4eeca44ecab48a66956acbb91d}, composed of left-hand X-ray images of the patient and their gender and age ($0$ to $20$ years). 
We alter the brightness of the X-ray images by a factor between $0$ and $6.5$ and form $20$ different NAS datasets to reflect the X-ray imaging set-ups in different hospitals following~\cite{Park2021NaturalAS}.
In-distribution data consists of images with a brightness factor $1.0$.
\edit{We trained a ResNet18 model using the cross-entropy loss and assessed it on the ID test set composed of images with a brightness factor of $1.0$.}
Further, we evaluate the NAS detection performance of our method and compare it with representative task-specific OOD detection methods on NAS datasets. Extensive details on the experimental set-up are described in \cref{sec:supp_experimental_details}.
For NAS detection, we measure the area under the receiver operating characteristic curve (AUROC), a commonly used metric for OOD detection. Additionally, we report the area under the precision-recall curve (AUPR) and the false positive rate of OOD examples when the true positive rate of in-distribution examples is at $95$\% (FPR95) in \cref{sec:supp_other_metrics}.}
 
% \vspace{-2mm}
\parahead{Results} The in-distribution classification accuracy
averaged across $10$ seeds 
of the gender classifier trained using cross-entropy loss
is $91.60$. We compare the NAS detection performance of our proposed approach with competitive post-hoc OOD detection methods in literature in \cref{tab:binary_class_nas}. \edit{As expected, the NAS detection performance of our approach and all baselines except KL Matching increase as the shift in the brightness attribute increases.}
We also observe that our proposed approaches, \emph{TAPUDD} and \emph{TAP-Mahalanobis} are more sensitive to NAS samples compared to competitive baselines, including Maximum Softmax Probability~\cite{hendrycks2017base}, ODIN~\cite{liang2017enhancing}, Mahalanobis distance~\cite{mahala18}, energy score~\cite{liu2020energy}, Gram matrices~\cite{sastry2021gram}, MOS~\cite{Huang2021MOSTS}, and  KL matching~\cite{Hendrycks2019ABF}. All these \edit{task-specific} baselines require the label information of the training dataset for OOD detection and cannot be used directly in tasks other than classification.
On the other hand, our proposed \edit{task-agnostic} approach does not require the access to class label information and it can be used across different tasks like regression. 

\subsection{NAS Detection in Regression}
\label{sec:regression_experiments}

\parahead{Experimental Details}
We use the RSNA Bone Age dataset (described in \cref{sec:binary_classification_experiments}) and solve the age prediction task. In this task, the objective is to automatically predict the patient's age given a hand X-ray image as an input.
\edit{As described in \cref{sec:binary_classification_experiments},}
we vary the brightness of images by a factor between $0$ and $6.5$ and form $20$ different NAS datasets.
In-distribution data comprises images of brightness factor $1.0$ (unmodified images).
We train a ResNet18 with MSE loss
and evaluate it on the test set composed of images with a brightness factor $1.0$.
Further, we evaluate the NAS detection performance of our proposed method and compare its performance with representative bayesian and non-bayesian uncertainty estimation methods on NAS datasets with attribute shift of brightness. Additionally, we compare the NAS detection performance of our approach with a well-known bayesian approach for uncertainty estimation, SWAG~\cite{maddox_2019_simple}. Extensive details on the experimental set-up are described in \cref{sec:supp_experimental_details}.
For NAS detection, we measure AUROC and additionally report AUPR and FPR95 in \cref{sec:supp_other_metrics}.

\begin{figure*}[hbt]
\vspace{-1.5mm}
\centering
     \includegraphics[width=0.82\textwidth]{wacv/main_paper/figures/experiments/pca.pdf}
    %  \vspace{-1mm}
     \caption{
     \edit{\emph{\textbf{(first row)}} Examples of ID images sampled from Imagenet and OOD images sampled from iNaturalist, SUN, Places, and Textures datasets; \emph{\textbf{(second row)}} Point-density based PCA visualization to demonstrate the location and density of ID and OOD datasets; \emph{\textbf{(third row)}} Point-density based PCA visualization of ID dataset overlapped by PCA of  OOD datasets to illustrate the location and density of OOD datasets relative to the ID dataset. \emph{\textbf{(fourth row)}} From \emph{\textbf{first}} and \emph{\textbf{third row}}, the key analysis is that \textbf{Textures is more OOD from Imagenet than the other three OOD datasets}.}}
     \label{fig:density_pca_ood_detection_final}
\end{figure*}

\input{wacv/main_paper/tables/multi_class_ood_detection}

% \vspace{2pt}
\parahead{Results} The in-distribution Mean Absolute Error (MAE) in year averaged across $10$ seeds of the Resnet18 model trained using MSE loss is $0.801$. We compare the NAS detection performance of our proposed approach with well-known uncertainty estimation methods, namely  Deep Ensemble (DE) ~\cite{lakshminarayanan2017simple}, Monte Carlo Dropout (MC Dropout) ~\cite{gal2016dropout}, and SWAG~\cite{maddox_2019_simple}. Although Deep Ensemble, MC Dropout, and SWAG are not applicable to a pre-trained model, we compare against these baselines as a benchmark, as it has shown strong OOD detection performance across regression examples. For DE, we retrain $10$ models of the same architecture (Resnet18) using MSE loss from different initializations.  Since SWAG is not directly applicable for OOD detection, we apply  $\text{SWAG}^{*}$ which is a combination of deep ensembling on top of SWAG. 
From \cref{tab:regression_nas}, \redit{as expected, we observe that the NAS detection performance of our approach and all baselines increase as the shift in the brightness attribute increases.}
We also observe that our proposed approaches, TAPUDD and \emph{TAP-Mahalanobis}, are more sensitive to NAS samples and effectively detect them compared to the baselines and TAP-MOS. 
Additionally, it can be seen that TAP-MOS fails to detect extremely dark samples (Brightness Intensity $0.1$). This might be because these NAS samples could locate near or 
% far away from the corner 
away from the periphery of all
clusters where MOS does not work well (as discussed in \cref{sec:synthetic_dataset_experiments}).
This demonstrates that our proposed approach is better than the existing approaches.


\begin{figure*}[t]
% \vspace{-2mm}
\centering
     \includegraphics[width=\textwidth]{wacv/main_paper/figures/experiments/ablations/ablation_clusters.pdf}
     \vspace{-4mm}
     \caption{Effect on OOD detection performance by using different number of clusters in \emph{TAP-Mahalanobis}.}
     \label{fig:cluster_ablation}
     \vspace{2mm}
\end{figure*}

\begin{figure*}[t]
% \vspace{-2mm}
\centering
     \includegraphics[width=\textwidth]{wacv/main_paper/figures/experiments/ablations/ablation_ensemble.pdf}
     \vspace{-4mm}
     \caption{Comparison of OOD detection performance of TAPUDD under different ensembling strategies. 
     }
    %  \vspace{-1mm}
     \label{fig:ensemble_ablation}
\end{figure*}

\subsection{OOD Detection for Large-scale Classification}
\label{sec:multi_classification_experiments}


% \vspace{-0.52mm}
\parahead{Experimental Details}
We use ImageNet-1k\cite{Deng2009ImageNetAL}
as the in-distribution dataset and evaluate our approach on diverse OOD datasets presented in MOS\cite{Huang2021MOSTS}, including iNaturalist\cite{Horn2018TheIS}, Places\cite{Zhou2018PlacesA1}, SUN\cite{sun2014deep}, and Textures\cite{Cimpoi2014DescribingTI}. 
For all baselines, we follow the experimental setup used in MOS\cite{Huang2021MOSTS}.
We obtained the base model for our approach by following the experimental setting of finetuning the fully connected layer \redit{of pretrained ResNetv2-101 model} by flattened softmax used in MOS.
We measure AUROC and FPR95 and report AUPR in \cref{sec:supp_other_metrics}.


\parahead{Analysis}
\edit{In binary classification (\cref{sec:binary_classification_experiments}) and regression (\cref{sec:regression_experiments}) tasks, we evaluated our approach on NAS samples and knew that the NAS detection performance should increase with the increase in attribute shift.
However, in this experiment, since the shift does not increase in a continuous manner, 
it is non-trivial to determine
for which OOD datasets scores should be high.
To this end, we perform an analysis wherein
from the \emph{\textbf{first row}} of \cref{fig:density_pca_ood_detection_final}, we observe that the Textures dataset is visually much more different to human eyes from Imagenet compared to the other three OOD datasets. }
\edit{
Further, in the \emph{\textbf{second}} and \emph{\textbf{third rows}} of \cref{fig:density_pca_ood_detection_final}, we apply principal component analysis (PCA) on the feature representations obtained from the penultimate layer of the model to visualize the location of in-distribution samples (Imagenet) and diverse OOD datasets. From this, we observe that most of the samples from the Textures dataset are located away from the highly-dense regions of Imagenet compared to the other three datasets, thus indicating that Textures is more OOD. 
Hence, \textit{\textbf{we expect a reliable OOD detection model to detect Textures as more OOD than the other three OOD datasets}}. 
}

% \vspace{-0.5mm}
\parahead{Results}
\edit{To determine the OOD detection methods that follow the expected analysis, we evaluate the performance of our approach and well-known post-hoc OOD detection methods, including
Maximum Softmax Probability~\cite{hendrycks2017base}, ODIN~\cite{liang2017enhancing}, Mahalanobis distance ~\cite{mahala18}, energy score ~\cite{liu2020energy},  MOS~\cite{Huang2021MOSTS}, and  KL matching~\cite{Hendrycks2019ABF}. It is also worth noting that all the baselines require class label information for OOD detection and cannot be used for tasks other than classification. 
From \cref{table:multi_class_ood}, we observe that only our approach (TAPUDD) and Mahalanobis follow the expected results, as highlighted in \textcolor{ForestGreen}{green} color. This demonstrates that all baselines except Mahalanobis are less reliable.
Further, we compare the performance of methods following the expected results (rows highlighted in \textcolor{ForestGreen}{green} color) and observe that \textbf{\textit{our approach (TAPUDD) is more sensitive to OOD samples and outperforms the baselines in all OOD datasets}}.}


\subsection{Ablations}
\label{sec:ablations}

\parahead{Effect of Number of Clusters in TAP-Mahalanobis}
% We investigate the effect of the number of clusters in the OOD detection performance of \emph{TAP-Mahalanobis} in \cref{fig:cluster_ablation}.
\edit{We investigate the effect of the number of clusters on the OOD detection performance of \emph{TAP-Mahalanobis} in \cref{fig:cluster_ablation}.}
We observe that the performance of \emph{TAP-Mahalanobis} varies with the value of K (\ie, number of clusters) across different datasets and tasks. This implies that we cannot use a particular value of K for all tasks and datasets.

% \vspace{1pt}
\parahead{TAPUDD with Different Ensembling Strategies}
We contrast the OOD detection performance of TAPUDD under different ensembling strategies for the three tasks in \cref{fig:ensemble_ablation}. We observe that TAPUDD shows competitive performance with diverse ensembling strategies for all the tasks and dataset shifts. Also, we observe that \quotes{seesaw} is slightly more sensitive towards NAS samples in binary classification and regression, and towards OOD samples from Places and SUN in large-class classification. 
 
Further, \cref{fig:cluster_ablation} and \cref{fig:ensemble_ablation} illustrate that using ensembling strategies provides us with an OOD detector which is almost as good as the best performer of \emph{TAP-Mahalanobis}.

\edit{We also evaluate our approach on other conventional OOD datasets (ID: CIFAR-10; OOD: CIFAR-100, SVHN, etc) and for anomaly detection task in  \cref{sec:cifar_level} and \cref{sec:anomaly_detection}, respectively.}
\editr{Additionally, we provide a 
% detailed
discussion on
% on the choice of GMM clustering in TAPUDD and 
tuning of hyperparameters in \cref{sec:discussion}.}

==> WACV 2023_ Task-Agnostic OOD Detection_arxiv/wacv/main_paper/sections/05_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this work, we propose a task-agnostic and post-hoc approach, TAPUDD, to detect samples from the unseen distribution. \editr{TAPUDD is a clustering-based ensembling approach 
% that utilizes the features from the trained model and is 
composed of \emph{TAP-Mahalanobis} and \emph{Ensembling} modules.} \emph{TAP-Mahalanobis} module groups the semantically similar training samples into clusters
% . At inference time, it 
\editr{and determines the minimum Mahalanobis distance of the test sample from the clusters.}  
\edit{To enhance reliability and to eliminate the necessity to determine the optimal number of clusters for \emph{TAP-Mahalanobis}, the \emph{Ensembling} module aggregates the distances obtained from the \emph{TAP-Mahalanobis} module for different values of clusters.}
\editr{We validate the effectiveness of our approach by conducting extensive experiments on diverse datasets and tasks.}
% We evaluate our approach 
% on synthetic and real-world datasets across diverse tasks and observe that our method effectively detects unseen samples. Further, we conducted ablation studies to analyze the effect of using different number of clusters and \emph{Ensembling} strategies in our approach. 
\edit{As future work, it would be interesting to extensively evaluate TAPUDD to detect samples from unseen distribution in natural language processing, 3D vision, and healthcare.}

==> WACV 2023_ Task-Agnostic OOD Detection_arxiv/wacv/main_paper/tables/binary_class_nas_detection.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\vspace{-0.2mm}
\small
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c  c  c  c c c  c c c c c }
\toprule
\multicolumn{1}{c}{\multirow{1}{*}{Brightness}} 
& \multicolumn{7}{c}{\multirow{1}{*}{Baselines}}  & \multicolumn{3}{c}{\multirow{1}{*}{Ours (Task-Agnostic)}} \\  \cmidrule(lr){2-8}  \cmidrule(lr){9-11} 
\multicolumn{1}{c}{} & \multicolumn{1}{c}{MSP~\cite{hendrycks2017base} } & \multicolumn{1}{c}{ODIN~\cite{liang2017enhancing} } & \multicolumn{1}{c}{Energy~\cite{liu2020energy} } & \multicolumn{1}{c}{MB~\cite{mahala18} } &  \multicolumn{1}{c}{KL~\cite{Hendrycks2019ABF} } &  \multicolumn{1}{c}{MOS~\cite{Huang2021MOSTS} } & \multicolumn{1}{c}{Gram~\cite{sastry2021gram}}  & \multicolumn{1}{c}{TAP-MOS} & \multicolumn{1}{c}{TAP-MB} & \multicolumn{1}{c}{TAPUDD} \\
& & & & & & (K = 8) & & (K = 8) & (K = 8) & (Average) 

\\ \midrule
        
0.0 & 88.7{\scriptsize $\pm$4.8} & 88.7{\scriptsize $\pm$4.8} & 88.2{\scriptsize $\pm$5.3} & 99.9{\scriptsize $\pm$0.1} & 26.3{\scriptsize $\pm$32.8} & 89.3{\scriptsize $\pm$5.5} & 99.3{\scriptsize $\pm$1.4} & 63.1{\scriptsize $\pm$26}   & 99.9{\scriptsize $\pm$0.1} & 100.0{\scriptsize $\pm$0.1} \\
% 0.1 & 83.2{\scriptsize $\pm$4}   & 83.2{\scriptsize $\pm$4}   & 83.1{\scriptsize $\pm$4.2} & 97.8{\scriptsize $\pm$1.2} & 34.9{\scriptsize $\pm$6.2}  & 83.1{\scriptsize $\pm$4.3} & 82.1{\scriptsize $\pm$7.7} & 74.2{\scriptsize $\pm$14.5} & 97.6{\scriptsize $\pm$2}   & 97.7{\scriptsize $\pm$2}   \\
0.2 & 66.1{\scriptsize $\pm$3.5} & 66.1{\scriptsize $\pm$3.5} & 66.0{\scriptsize $\pm$3.7}   & 87.5{\scriptsize $\pm$4.5} & 44.5{\scriptsize $\pm$3}    & 65.9{\scriptsize $\pm$3.2} & 61.0{\scriptsize $\pm$3.3}   & 63.6{\scriptsize $\pm$10}   & 86.8{\scriptsize $\pm$4.7} & 87.3{\scriptsize $\pm$5.2} \\
% 0.3 & 59.5{\scriptsize $\pm$2}   & 59.6{\scriptsize $\pm$2}   & 59.4{\scriptsize $\pm$2.4} & 77.7{\scriptsize $\pm$4.6} & 46.9{\scriptsize $\pm$1.5}  & 59.5{\scriptsize $\pm$1.6} & 55.5{\scriptsize $\pm$1.6} & 58.8{\scriptsize $\pm$6.8}  & 76.6{\scriptsize $\pm$4.1} & 77.2{\scriptsize $\pm$5.1}  \\
0.4 & 56.3{\scriptsize $\pm$1.4} & 56.4{\scriptsize $\pm$1.4} & 56.2{\scriptsize $\pm$1.7} & 70.5{\scriptsize $\pm$3.8} & 46.9{\scriptsize $\pm$1.2}  & 56.4{\scriptsize $\pm$1.1} & 53.4{\scriptsize $\pm$1.1} & 56.3{\scriptsize $\pm$4.9}  & 69.6{\scriptsize $\pm$3.7} & 70.1{\scriptsize $\pm$4.5}\\
% 0.5 & 54{\scriptsize $\pm$1}     & 54{\scriptsize $\pm$1}     & 53.9{\scriptsize $\pm$1.2} & 64.6{\scriptsize $\pm$3.2} & 47.7{\scriptsize $\pm$0.9}  & 54.1{\scriptsize $\pm$0.9} & 52.2{\scriptsize $\pm$0.8} & 54.3{\scriptsize $\pm$3.4}  & 63.8{\scriptsize $\pm$3.2} & 64.1{\scriptsize $\pm$3.7} \\
0.6 & 52.4{\scriptsize $\pm$0.8} & 52.4{\scriptsize $\pm$0.8} & 52.3{\scriptsize $\pm$0.9} & 59.9{\scriptsize $\pm$2.5} & 48.2{\scriptsize $\pm$1}    & 52.5{\scriptsize $\pm$0.8} & 51.4{\scriptsize $\pm$0.5} & 52.7{\scriptsize $\pm$2.4}  & 59.3{\scriptsize $\pm$2.5} & 59.4{\scriptsize $\pm$2.7} \\
% 0.7 & 51.3{\scriptsize $\pm$0.6} & 51.3{\scriptsize $\pm$0.6} & 51.2{\scriptsize $\pm$0.6} & 55.7{\scriptsize $\pm$2}   & 48.5{\scriptsize $\pm$0.7}  & 51.4{\scriptsize $\pm$0.6} & 50.8{\scriptsize $\pm$0.5} & 51.4{\scriptsize $\pm$1.7}  & 55.4{\scriptsize $\pm$2.2} & 55.4{\scriptsize $\pm$2.2} \\
0.8 & 50.4{\scriptsize $\pm$0.4} & 50.4{\scriptsize $\pm$0.4} & 50.4{\scriptsize $\pm$0.4} & 52.2{\scriptsize $\pm$1.4} & 48.8{\scriptsize $\pm$0.6}  & 50.5{\scriptsize $\pm$0.3} & 50.2{\scriptsize $\pm$0.5} & 50.5{\scriptsize $\pm$1.2}  & 52.0{\scriptsize $\pm$1.7}   & 52.0{\scriptsize $\pm$1.6}   \\
% 0.9 & 50{\scriptsize $\pm$0.2}   & 50{\scriptsize $\pm$0.2}   & 50{\scriptsize $\pm$0.2}   & 50.1{\scriptsize $\pm$0.7} & 49.5{\scriptsize $\pm$0.4}  & 50{\scriptsize $\pm$0.2}   & 50.1{\scriptsize $\pm$0.4} & 50{\scriptsize $\pm$0.6}    & 50{\scriptsize $\pm$0.8}   & 50{\scriptsize $\pm$0.7}    \\
 \rowcolor{Gray} 1.0 & 50.0{\scriptsize $\pm$0.0}     & 50.0{\scriptsize $\pm$0.0}     & 50.0{\scriptsize $\pm$0.0}     & 50.0{\scriptsize $\pm$0.0}     & 50.0{\scriptsize $\pm$0.0}      & 50.0{\scriptsize $\pm$0.0}     & 50.0{\scriptsize $\pm$0.0}     & 50.0{\scriptsize $\pm$0.0}      & 50.0{\scriptsize $\pm$0.0}     & 50.0{\scriptsize $\pm$0.0}     \\
% 1.1 & 50.5{\scriptsize $\pm$0.2} & 50.5{\scriptsize $\pm$0.2} & 50.5{\scriptsize $\pm$0.2} & 51.9{\scriptsize $\pm$0.6} & 49.8{\scriptsize $\pm$0.4}  & 50.5{\scriptsize $\pm$0.2} & 50.3{\scriptsize $\pm$0.5} & 50.4{\scriptsize $\pm$0.5}  & 52{\scriptsize $\pm$0.6}   & 52{\scriptsize $\pm$0.5}  \\
1.2 & 51.7{\scriptsize $\pm$0.4} & 51.7{\scriptsize $\pm$0.4} & 51.7{\scriptsize $\pm$0.4} & 55.4{\scriptsize $\pm$1.6} & 49.2{\scriptsize $\pm$0.5}  & 51.7{\scriptsize $\pm$0.5} & 51.1{\scriptsize $\pm$0.6} & 51.2{\scriptsize $\pm$0.9}  & 56.1{\scriptsize $\pm$1.5} & 56.0{\scriptsize $\pm$1.5}    \\
% 1.3 & 53.5{\scriptsize $\pm$0.6} & 53.5{\scriptsize $\pm$0.6} & 53.6{\scriptsize $\pm$0.6} & 59.5{\scriptsize $\pm$1.9} & 48.8{\scriptsize $\pm$0.8}  & 53.5{\scriptsize $\pm$0.7} & 52.2{\scriptsize $\pm$0.9} & 52.3{\scriptsize $\pm$1.4}  & 60.1{\scriptsize $\pm$2}   & 60{\scriptsize $\pm$1.9}   \\
1.4 & 55.8{\scriptsize $\pm$0.8} & 55.8{\scriptsize $\pm$0.8} & 55.8{\scriptsize $\pm$0.8} & 62.9{\scriptsize $\pm$2.1} & 48.2{\scriptsize $\pm$1.2}  & 55.8{\scriptsize $\pm$0.8} & 53.6{\scriptsize $\pm$1.1} & 53.6{\scriptsize $\pm$1.7}  & 63.7{\scriptsize $\pm$2.0}   & 63.5{\scriptsize $\pm$2.1} \\
% 1.5 & 57.9{\scriptsize $\pm$1}   & 57.9{\scriptsize $\pm$1}   & 58{\scriptsize $\pm$1.1}   & 66.4{\scriptsize $\pm$2.3} & 47.5{\scriptsize $\pm$1.3}  & 57.9{\scriptsize $\pm$1}   & 54.8{\scriptsize $\pm$1.1} & 54.9{\scriptsize $\pm$2}    & 67.2{\scriptsize $\pm$2.3} & 67{\scriptsize $\pm$2.4}  \\
1.6 & 59.7{\scriptsize $\pm$1.3} & 59.7{\scriptsize $\pm$1.3} & 59.8{\scriptsize $\pm$1.4} & 70.2{\scriptsize $\pm$2.7} & 47.5{\scriptsize $\pm$1.7}  & 59.6{\scriptsize $\pm$1.1} & 55.9{\scriptsize $\pm$1.2} & 55.8{\scriptsize $\pm$2.4}  & 70.9{\scriptsize $\pm$2.8} & 70.7{\scriptsize $\pm$2.9}   \\
% 1.7 & 61.5{\scriptsize $\pm$1.7} & 61.5{\scriptsize $\pm$1.7} & 61.6{\scriptsize $\pm$1.8} & 73.6{\scriptsize $\pm$2.9} & 47.9{\scriptsize $\pm$2.1}  & 61.3{\scriptsize $\pm$1.4} & 57.1{\scriptsize $\pm$1.4} & 56.5{\scriptsize $\pm$3.1}  & 74.2{\scriptsize $\pm$3.1} & 73.9{\scriptsize $\pm$3.3}  \\
1.8 & 63.1{\scriptsize $\pm$2.0}   & 63.1{\scriptsize $\pm$2.1} & 63.2{\scriptsize $\pm$2.2} & 76.5{\scriptsize $\pm$2.9} & 48.3{\scriptsize $\pm$2.4}  & 62.8{\scriptsize $\pm$1.7} & 58.1{\scriptsize $\pm$1.5} & 57.0{\scriptsize $\pm$4.0}      & 76.9{\scriptsize $\pm$3.4} & 76.6{\scriptsize $\pm$3.5} \\
% 1.9 & 64.4{\scriptsize $\pm$2.7} & 64.4{\scriptsize $\pm$2.7} & 64.5{\scriptsize $\pm$2.9} & 79.1{\scriptsize $\pm$2.9} & 49{\scriptsize $\pm$2.8}    & 64.1{\scriptsize $\pm$2.1} & 59.3{\scriptsize $\pm$1.7} & 57.4{\scriptsize $\pm$5.1}  & 79.5{\scriptsize $\pm$3.6} & 79.1{\scriptsize $\pm$3.7}  \\
2.0 & 65.5{\scriptsize $\pm$3.2} & 65.6{\scriptsize $\pm$3.2} & 65.7{\scriptsize $\pm$3.5} & 81.6{\scriptsize $\pm$2.7} & 49.8{\scriptsize $\pm$2.9}  & 65.1{\scriptsize $\pm$2.6} & 60.5{\scriptsize $\pm$1.8} & 57.7{\scriptsize $\pm$6.0}    & 81.8{\scriptsize $\pm$3.7} & 81.4{\scriptsize $\pm$3.8} \\
2.5 & 69.5{\scriptsize $\pm$6.5} & 69.5{\scriptsize $\pm$6.5} & 69.6{\scriptsize $\pm$6.8} & 90.4{\scriptsize $\pm$2.5} & 51.6{\scriptsize $\pm$4.9}  & 69.0{\scriptsize $\pm$5.5}   & 65.4{\scriptsize $\pm$4.4} & 60.0{\scriptsize $\pm$9.0}      & 89.9{\scriptsize $\pm$3.8} & 89.6{\scriptsize $\pm$4.1} \\
3.0 & 72.5{\scriptsize $\pm$8.7} & 72.5{\scriptsize $\pm$8.7} & 72.6{\scriptsize $\pm$9.0}   & 94.8{\scriptsize $\pm$1.8} & 51.3{\scriptsize $\pm$5.4}  & 72.0{\scriptsize $\pm$7.6}   & 69.6{\scriptsize $\pm$5.9} & 63.0{\scriptsize $\pm$11.5}   & 93.9{\scriptsize $\pm$3.8} & 93.6{\scriptsize $\pm$4.0}  \\
3.5 & 73.7{\scriptsize $\pm$9.7} & 73.7{\scriptsize $\pm$9.7} & 73.6{\scriptsize $\pm$10}  & 96.8{\scriptsize $\pm$1.3} & 52.0{\scriptsize $\pm$6.1}    & 73.0{\scriptsize $\pm$8.8}   & 72.2{\scriptsize $\pm$6.8} & 64.3{\scriptsize $\pm$13.6} & 95.5{\scriptsize $\pm$3.8} & 95.4{\scriptsize $\pm$3.7} \\
4.0 & 75.8{\scriptsize $\pm$9.5} & 75.8{\scriptsize $\pm$9.5} & 75.7{\scriptsize $\pm$9.8} & 97.8{\scriptsize $\pm$0.8} & 50.5{\scriptsize $\pm$7.2}  & 75.3{\scriptsize $\pm$8.8} & 75.1{\scriptsize $\pm$7.9} & 66.3{\scriptsize $\pm$14.4} & 96.5{\scriptsize $\pm$3.6} & 96.5{\scriptsize $\pm$3.2} \\
4.5 & 78.1{\scriptsize $\pm$7.9} & 78.1{\scriptsize $\pm$7.9} & 78.0{\scriptsize $\pm$8.3}   & 98.5{\scriptsize $\pm$0.5} & 47.4{\scriptsize $\pm$8.2}  & 77.8{\scriptsize $\pm$7.5} & 78.0{\scriptsize $\pm$7.1}   & 68.7{\scriptsize $\pm$13.7} & 97.3{\scriptsize $\pm$3.0}   & 97.4{\scriptsize $\pm$2.4}   \\
5.0 & 79.9{\scriptsize $\pm$6.4} & 79.9{\scriptsize $\pm$6.4} & 79.8{\scriptsize $\pm$6.9} & 98.8{\scriptsize $\pm$0.4} & 44.9{\scriptsize $\pm$8.4}  & 79.8{\scriptsize $\pm$6.1} & 80.4{\scriptsize $\pm$6.6} & 70.3{\scriptsize $\pm$12.8} & 97.9{\scriptsize $\pm$2.5} & 98.0{\scriptsize $\pm$1.7}    \\
5.5 & 81.4{\scriptsize $\pm$5.6} & 81.4{\scriptsize $\pm$5.6} & 81.3{\scriptsize $\pm$6.2} & 99.0{\scriptsize $\pm$0.4}   & 44.1{\scriptsize $\pm$8.7}  & 81.3{\scriptsize $\pm$5.4} & 82.4{\scriptsize $\pm$6.6} & 71.3{\scriptsize $\pm$12.7} & 98.2{\scriptsize $\pm$2.2} & 98.4{\scriptsize $\pm$1.2}   \\
6.0 & 82.5{\scriptsize $\pm$5.1} & 82.5{\scriptsize $\pm$5.1} & 82.5{\scriptsize $\pm$5.6} & 99.1{\scriptsize $\pm$0.4} & 43.6{\scriptsize $\pm$8.6}  & 82.4{\scriptsize $\pm$4.9} & 83.9{\scriptsize $\pm$6.3} & 71.9{\scriptsize $\pm$12.8} & 98.5{\scriptsize $\pm$1.9} & 98.7{\scriptsize $\pm$0.9}  \\
6.5 & 83.2{\scriptsize $\pm$4.9} & 83.2{\scriptsize $\pm$4.9} & 83.2{\scriptsize $\pm$5.4} & 99.2{\scriptsize $\pm$0.4} & 44.3{\scriptsize $\pm$8.2}  & 83.1{\scriptsize $\pm$4.6} & 85.0{\scriptsize $\pm$6.2}   & 72.2{\scriptsize $\pm$13.1} & 98.7{\scriptsize $\pm$1.7} & 98.9{\scriptsize $\pm$0.7}  \\
% 7.0 & 83.6{\scriptsize $\pm$4.7} & 83.6{\scriptsize $\pm$4.7} & 83.6{\scriptsize $\pm$5.2} & 99.2{\scriptsize $\pm$0.4} & 44.5{\scriptsize $\pm$8}    & 83.4{\scriptsize $\pm$4.5} & 85.6{\scriptsize $\pm$6.2} & 72.2{\scriptsize $\pm$13.4} & 98.8{\scriptsize $\pm$1.5} & 99{\scriptsize $\pm$0.6}   \\
% 7.5 & 83.6{\scriptsize $\pm$4.8} & 83.6{\scriptsize $\pm$4.8} & 83.6{\scriptsize $\pm$5.3} & 99.3{\scriptsize $\pm$0.4} & 44.8{\scriptsize $\pm$8.2}  & 83.4{\scriptsize $\pm$4.7} & 85.8{\scriptsize $\pm$6.4} & 71.8{\scriptsize $\pm$14}   & 98.9{\scriptsize $\pm$1.4} & 99.1{\scriptsize $\pm$0.5} \\
\midrule
Average & 67.8 & 67.8 & 67.8 & 82.1 & 46.9 & 67.7   & 66.8 & 61.0 & \textbf{81.7 }& \textbf{82.0 } \\
 \bottomrule
 \end{tabular}}
%  \vspace{-2mm}
\vspace{0.1mm}
\caption{NAS detection performance in binary classification task for NAS shift of brightness in RSNA boneage dataset measured by AUROC. Highlighted row presents the performance on ID data. MB and TAP-MB refers to Mahalanobis and \emph{TAP-Mahalanobis}, respectively.
\edit{Our task-agnostic approach significantly outperforms all baselines (except MB) and is comparable to MB. Note that \textbf{MB is task-specific} and cannot be used in tasks other than classification.}
}
\label{tab:binary_class_nas}
% \vspace{-1mm}
\end{table*}
        

==> WACV 2023_ Task-Agnostic OOD Detection_arxiv/wacv/main_paper/tables/multi_class_nas_detection.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\footnotesize
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c c c  c  c  c c c  c c c}
\toprule
&\multicolumn{1}{c}{\multirow{1}{*}{Distribution}} & \multicolumn{1}{c}{\multirow{1}{*}{Brightness}} 
& \multicolumn{6}{c}{\multirow{1}{*}{Baselines}}  & \multicolumn{2}{c}{\multirow{1}{*}{Ours}} \\ \cmidrule(lr){4-9}  \cmidrule(lr){10-11} 
&\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{MSP~\cite{hendrycks2017base} } & \multicolumn{1}{c}{ODIN~\cite{liang2017enhancing} } & \multicolumn{1}{c}{Energy~\cite{liu2020energy} } & \multicolumn{1}{c}{MB~\cite{mahala18} } &  \multicolumn{1}{c}{KL~\cite{Hendrycks2019ABF} } &  \multicolumn{1}{c}{MOS~\cite{Huang2021MOSTS} } & \multicolumn{1}{c}{K = 32} & \multicolumn{1}{c}{K = 8}  

\\ \midrule
\parbox[t]{2mm}{\multirow{32}{*}{\rotatebox[origin=c]{90}{RSNA Bone Age}}}

 & \multirow{10}{*}{NAS} & 0.0 & 99.98 & 100.00 & 100.00 & 100.00 & 84.36 & 85.29 & 100.00 & 100.00 \\
 &  & 0.1 & 80.60 & 83.72 & 83.94 & 92.46 & 76.61 & 76.61 & 84.69 & 80.04 \\
 &  & 0.2 & 72.78 & 75.46 & 75.42 & 84.77 & 69.97 & 70.23 & 75.68 & 71.57 \\
 &  & 0.3 & 69.53 & 71.88 & 71.75 & 77.86 & 67.10 & 67.26 & 70.56 & 66.71 \\
 &  & 0.4 & 67.91 & 70.05 & 69.88 & 72.84 & 65.71 & 65.80 & 67.10 & 63.42 \\
 &  & 0.5 & 66.98 & 68.97 & 68.77 & 69.68 & 64.92 & 65.04 & 64.65 & 61.10 \\
 &  & 0.6 & 66.45 & 68.36 & 68.14 & 66.99 & 64.44 & 64.63 & 62.84 & 59.41 \\
 &  & 0.7 & 66.10 & 67.95 & 67.73 & 64.68 & 64.16 & 64.43 & 61.63 & 58.32 \\
 &  & 0.8 & 65.90 & 67.72 & 67.49 & 62.26 & 64.00 & 64.36 & 60.94 & 57.74 \\
 &  & 0.9 & 65.80 & 67.60 & 67.37 & 59.66 & 63.95 & 64.35 & 60.64 & 57.52 \\ \cdashline{2-11}[1pt/1pt]
 & ID & 1.0 & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 \\ \cdashline{2-11}[1pt/1pt]
 & \multirow{21}{*}{NAS} & 1.1 & 65.98 & 67.84 & 67.62 & 54.88 & 64.05 & 64.55 & 60.50 & 57.33 \\
 &  & 1.2 & 66.50 & 68.49 & 68.31 & 53.74 & 64.41 & 64.99 & 60.63 & 57.25 \\
 &  & 1.3 & 67.21 & 69.37 & 69.22 & 53.29 & 64.95 & 65.60 & 60.96 & 57.33 \\
 &  & 1.4 & 68.10 & 70.44 & 70.33 & 53.39 & 65.65 & 66.37 & 61.48 & 57.56 \\
 &  & 1.5 & 69.09 & 71.60 & 71.53 & 53.94 & 66.47 & 67.21 & 62.15 & 57.91 \\
 &  & 1.6 & 70.13 & 72.79 & 72.76 & 54.67 & 67.37 & 68.08 & 62.90 & 58.34 \\
 &  & 1.7 & 71.19 & 74.00 & 74.02 & 55.56 & 68.33 & 68.99 & 63.71 & 58.82 \\
 &  & 1.8 & 72.27 & 75.20 & 75.25 & 56.55 & 69.36 & 69.88 & 64.57 & 59.35 \\
 &  & 1.9 & 73.33 & 76.35 & 76.44 & 57.51 & 70.41 & 70.76 & 65.41 & 59.88 \\
 &  & 2.0 & 74.42 & 77.50 & 77.62 & 58.59 & 71.50 & 71.66 & 66.29 & 60.43 \\
 &  & 2.5 & 78.99 & 82.19 & 82.42 & 63.02 & 76.20 & 75.50 & 69.95 & 62.74 \\
 &  & 3.0 & 82.50 & 85.61 & 85.90 & 66.94 & 79.95 & 78.58 & 72.99 & 64.75 \\
 &  & 3.5 & 85.08 & 88.06 & 88.41 & 70.06 & 82.73 & 81.02 & 75.54 & 66.54 \\
 &  & 4.0 & 87.06 & 89.90 & 90.29 & 72.70 & 84.86 & 83.03 & 77.76 & 68.19 \\
 &  & 4.5 & 88.53 & 91.24 & 91.67 & 74.73 & 86.49 & 84.64 & 79.66 & 69.70 \\
 &  & 5.0 & 89.70 & 92.30 & 92.76 & 76.51 & 87.74 & 86.02 & 81.36 & 71.12 \\
 &  & 5.5 & 90.57 & 93.10 & 93.58 & 77.92 & 88.69 & 87.16 & 82.81 & 72.41 \\
 &  & 6.0 & 91.27 & 93.74 & 94.26 & 79.20 & 89.47 & 88.16 & 84.11 & 73.65 \\
 &  & 6.5 & 91.81 & 94.24 & 94.79 & 80.21 & 90.08 & 88.99 & 85.23 & 74.76 \\
 &  & 7.0 & 92.24 & 94.66 & 95.24 & 81.14 & 90.60 & 89.73 & 86.26 & 75.83 \\
 &  & 7.5 & 92.57 & 94.98 & 95.60 & 81.90 & 91.04 & 90.37 & 87.16 & 76.79 \\
 \bottomrule
\end{tabular}}
\caption{NAS detection performance for multi-class classification task on distributional shifts in RSNA boneage dataset measured by AUROC. \radhika{1. add plots for comparison in supplementary}
% Mahala and Mahala* indicate using penultimate layer only or ensembling all layer respectively.
}
\label{tab:binary_class_nas}
% \vspace{-4mm}
\end{table*}

==> WACV 2023_ Task-Agnostic OOD Detection_arxiv/wacv/main_paper/tables/multi_class_ood_detection.tex <==
% \begin{table*}[ht]
% \footnotesize
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|c|cc|cc|cc|cc|cc}
% \toprule
% \multirow{3}{*}{\textbf{Method}} & \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Test \\ Time\\ (min)\end{tabular}}} & \multicolumn{2}{c|}{\textbf{iNaturalist}}    & \multicolumn{2}{c|}{\textbf{SUN}}            & \multicolumn{2}{c|}{\textbf{Places}}         & \multicolumn{2}{c|}{\textbf{Textures}}       & \multicolumn{2}{c}{\textbf{Average}}        \\ \cline{3-12} 
%                                  &                                                                                        & \textbf{AUROC}       & \textbf{FPR95}        & \textbf{AUROC}       & \textbf{FPR95}        & \textbf{AUROC}       & \textbf{FPR95}        & \textbf{AUROC}       & \textbf{FPR95}        & \textbf{AUROC}       & \textbf{FPR95}       \\
%                                  &                                                                                        & \multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c|}{$\downarrow$} & \multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c|}{$\downarrow$} & \multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c|}{$\downarrow$} & \multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c|}{$\downarrow$} & \multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c}{$\downarrow$}  \\ \midrule
% MSP~\cite{hendrycks2017base} & - & 87.70 & 63.52 & 78.22 & 80.01 & 76.67 & 81.31 & 74.46 & 82.70 & 79.26 & 76.88 \\
% ODIN~\cite{liang2017enhancing} & - & 89.49 & 62.61 & 83.83 & 71.89 & 80.60 & 76.51 & 76.29 & 81.31 & 82.55 & 73.08 \\
% M\cite{mahala18} & - & 59.60 & 95.62 & 67.96 & 91.58 & 66.48 & 92.05 & 74.96 & 51.54 & 67.25 & 82.70 \\
% Energy~\cite{liu2020energy} & - & 88.64 & 64.35 & 85.25 & 65.30 & 81.31 & 72.77 & 75.78 & 80.60 & 82.75 & 70.76 \\
% KL Matching~\cite{Hendrycks2019ABF} & - & 93.06 & 27.24 & 78.74 & 67.56 & 76.53 & 72.67 & 87.07 & 49.47 & 83.85 & 54.23 \\
% MOS~\cite{Huang2021MOSTS} & - & 98.15 & 9.23 & 92.01 & 40.38 & 89.05 & 49.49 & 81.27 & 60.30 & 90.12 & 39.85 \\ \midrule
% Ours (K = 5) & - & 70.51 & 79.55 & 73.40 & 77.07 & 70.22 & 82.05 & 96.58 & 15.46 & 77.68 & 63.53 \\
% Ours ( best/data) & - & 75.58 & 77.21 & 75.42 & 74.53 & 70.49 & 81.04 & 98.23 & 8.81 & 79.93 & 60.40 \\
% Ours (K = 8) & - & 69.59 & 83.50 & 71.98 & 77.99 & 69.47 & 82.71 & 95.39 & 18.35 & 76.61 & 65.64       \\ \bottomrule
% \end{tabular}

% }
% \caption{\small{OOD detection performance comparison between MOS and baselines. All methods are fine-tuned from the same pre-trained BiT-S-R101x1 backbone with ImageNet-1k as in-distribution dataset. The description of 4 OOD test datasets is provided in Section~\ref{sec:dataset}. $\uparrow$ indicates larger values are better, while $\downarrow$ indicates smaller values are better. All values are percentages. \textbf{Bold} numbers are superior results. Test time for all methods are evaluated with the same in- and out-of-distribution datasets (60k images in total). }} %\SL{add citations to baselines}}
% \label{table:main_result}
% \vspace{-0.3cm}
% \end{table*}

\begin{table*}[t]
% \vspace{-1mm}
\footnotesize
\centering
% \textcolor{ForestGreen}{\text{\normalsize{\textbf{Expected Tendency}: \textit{Higher AUROC/Lower FPR95 for Textures; Lower AUROC/Higher FPR95 for other three datasets.}}}}
% \textcolor{ForestGreen}{\text{\normalsize{\textbf{Expected Results}: \textit{Higher AUROC/Lower FPR95 for Textures; Lower AUROC/Higher FPR95 for other three datasets.}}}}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc}
\toprule
\multirow{3}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{iNaturalist}}    & \multicolumn{2}{c|}{\textbf{SUN}}            & \multicolumn{2}{c|}{\textbf{Places}}         & \multicolumn{2}{c|}{\textbf{Textures}}       & \multicolumn{2}{c}{\textbf{Average}}        \\ \cmidrule{2-11} 
                                 &                                                                                        \textbf{AUROC} $\uparrow$      & \textbf{FPR95} {$\downarrow$}       & \textbf{AUROC} $\uparrow$       & \textbf{FPR95} {$\downarrow$}         & \textbf{AUROC} $\uparrow$        & \textbf{FPR95} {$\downarrow$}         & \textbf{AUROC} $\uparrow$        & \textbf{FPR95} {$\downarrow$}         & \textbf{AUROC} $\uparrow$        & \textbf{FPR95} {$\downarrow$}        \\
                                 %&                                                                                        \multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c|}{$\downarrow$} & \multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c|}{$\downarrow$} & \multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c|}{$\downarrow$} & \multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c|}{$\downarrow$} & \multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c}{$\downarrow$}  \\ 
                                 \midrule
\rowcolor{teagreen} \textbf{Expected Results} & Low & High & Low & High & Low & High & \textbf{High} & \textbf{Low}  & -- & --  \\ \midrule
MSP~\cite{hendrycks2017base} & 87.70 & 63.52 & 78.22 & 80.01 & 76.67 & 81.31 & 74.46 & 82.70 & 79.26 & 76.88 \\
ODIN~\cite{liang2017enhancing} & 89.49 & 62.61 & 83.83 & 71.89 & 80.60 & 76.51 & 76.29 & 81.31 & 82.55 & 73.08 \\
\rowcolor{teagreen}Mahalanobis \cite{mahala18} & 59.60 & 95.62 & 67.96 & 91.58 & 66.48 & 92.05 & 74.96 & 51.54 & 67.25 & 82.70 \\
Energy~\cite{liu2020energy} & 88.64 & 64.35 & 85.25 & 65.30 & 81.31 & 72.77 & 75.78 & 80.60 & 82.75 & 70.76 \\
KL Matching~\cite{Hendrycks2019ABF} & 93.06 & 27.24 & 78.74 & 67.56 & 76.53 & 72.67 & 87.07 & 49.47 & 83.85 & 54.23 \\
MOS~\cite{Huang2021MOSTS} & 98.15 & 9.23 & 92.01 & 40.38 & 89.05 & 49.49 & 81.27 & 60.30 & 90.12 & 39.85 \\ \midrule
% \rowcolor{lightyellow} \textbf{TAP-MB (K = 5)} & \textbf{70.51} & \textbf{79.55} & \textbf{73.40} & \textbf{77.07} & \textbf{70.22} & \textbf{82.05} & 96.58 & 15.46 & \textbf{77.68} & \textbf{63.53} \\
% Ours (best/data) & 75.58 & 77.21 & 75.42 & 74.53 & 70.49 & 81.04 & \textbf{98.23} & \textbf{08.81} & 79.93 & 60.40 \\
% \rowcolor{lightyellow} \textbf{TAP-MB (K = 8)} & 69.59 & 83.50 & 71.98 & 77.99 & 69.47 & 82.71 & 95.39 & 18.35 & 76.61 & 65.64   \\ 
% \midrule
\rowcolor{teagreen}\textbf{TAPUDD (Average)} & \textbf{70.00} & \textbf{84.46} & \textbf{70.47 }& \textbf{79.52} & \textbf{66.97} & \textbf{84.72} & \textbf{97.59} & \textbf{10.85} & \textbf{76.26} & \textbf{64.88}  \\
% TAUOOD (Trimmed Average) & 70.18 & 83.53 & 71.12 & 78.28 & 67.70 & 83.61 & \textbf{97.35} & \textbf{12.04} & 76.59  & 64.36 \\
% TAUOOD (Seesaw) & 70.05 & 82.98 & 72.61 & 76.38 & 69.41 & 81.58 & \textbf{96.59} & \textbf{14.98} & 77.16 & 63.98 \\
% TAUOOD (Top) & 71.15 & 81.88 & 71.92 & 77.04 & 68.65 & 82.32 & \textbf{97.07} &\textbf{ 13.28 } & 77.19  & 63.63 \\
% TAUOOD (Bottom) & 69.17 & 85.89 & 69.70 & 80.61 & 66.09 & 85.81 & \textbf{97.69} & \textbf{10.41} & 75.66 & 65.68 \\
\bottomrule
\end{tabular}
}
\vspace{0.1mm}
\caption{
% \edit{OOD detection performance in the large-scale classification task.
% % TAP-MB denotes TAP-Mahalanobis.
% $\uparrow$ indicates larger values are better, while $\downarrow$ indicates smaller values are better. 
% Ideally, we expect all methods to follow the tendency obtained from our analysis (described in \textcolor{ForestGreen}{green} color).
% However, as highlighted in \colorbox{teagreen}{green} color, only Mahalanobis and our proposed approaches follow the desired tendency. This highlights the failure of existing baselines, including MSP, ODIN, Energy, KL Matching, and MOS.
% Further, amongst all methods following the desired tendency, \textbf{\textit{our approach is highly sensitive to OOD samples and significantly outperforms the baselines}}. 
\edit{OOD detection performance in the large-scale classification task.
% TAP-MB denotes TAP-Mahalanobis.
$\uparrow$ indicates larger values are better, while $\downarrow$ indicates smaller values are better. 
Ideally, all methods should follow the expected results obtained from our analysis (described in first row in \textcolor{ForestGreen}{green} color).
However, as highlighted in \textcolor{ForestGreen}{green} color, only Mahalanobis and our proposed approach follow the expected results. This highlights the failure of existing baselines, including MSP, ODIN, Energy, KL Matching, and MOS.
Further, amongst all methods following the expected results (highlighted in \textcolor{ForestGreen}{green} color), \textbf{\textit{our approach is highly sensitive to OOD samples and significantly outperforms the baselines}}. }
% In contrast to existing methods (except Mahalanobis), our method detects samples from the Textures dataset more OOD than samples from iNaturalist, SUN, and Places (similar to the way humans perceive). 
% This demonstrates the failure of existing methods. 
}
% \edit{TAP-MB denotes TAP-Mahalanobis.}
% % All methods are fine-tuned from the same pre-trained BiT-S-R101x1 backbone with ImageNet-1k as in-distribution dataset. 
% $\uparrow$ indicates larger values are better, while $\downarrow$ indicates smaller values are better. 
% %All values are in percentages and \textbf{Bold} numbers are superior results. 
% \edit{In contrast to existing methods except Mahalanobis, }our method detects samples from Textures dataset more OOD compared to samples from iNaturalist, SUN, Places (similar to the way humans perceive).  
% % All baselines except Mahalanobis detects samples from textures dataset less OOD compared to iNaturalist, SUN, and Places. 
% \edit{This demonstrates the failure of existing methods}.

\label{table:multi_class_ood}
% \vspace{-1mm}
\end{table*}

==> WACV 2023_ Task-Agnostic OOD Detection_arxiv/wacv/main_paper/tables/regression.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\vspace{-0.2mm}
% \begin{wraptable}{r}{13cm}
\footnotesize
\centering
\resizebox{0.76\linewidth}{!}{
\begin{tabular}{c  c  c  c c c  c }
\toprule
\multicolumn{1}{c}{\multirow{1}{*}{Brightness}} 
& \multicolumn{3}{c}{\multirow{1}{*}{Baselines}}  & \multicolumn{3}{c}{\multirow{1}{*}{Ours (Task-Agnostic)}} \\  \cmidrule(lr){2-4}  \cmidrule(lr){5-7} 
\multicolumn{1}{c}{} & \multicolumn{1}{c}{DE~\cite{lakshminarayanan2017simple} } & \multicolumn{1}{c}{MC Dropout~\cite{gal2016dropout} } & \multicolumn{1}{c}{$\text{SWAG}^{*}$~\cite{maddox_2019_simple}}  & \multicolumn{1}{c}{TAP-MOS} & \multicolumn{1}{c}{TAP-MB} & \multicolumn{1}{c}{TAPUDD}\\
& & & & (K = 8) & (K = 8) & (Average) 

\\ \midrule
0.0 &  100.0{\scriptsize $\pm$NA} & 6.9{\scriptsize $\pm$NA}& 99.9{\scriptsize $\pm$NA} & 57.8{\scriptsize $\pm$31.5} & 100.0{\scriptsize $\pm$0.1} & 100.0{\scriptsize $\pm$0.0} \\
0.2 & 57.0{\scriptsize $\pm$NA} & 45.5{\scriptsize $\pm$NA} & 51.4{\scriptsize $\pm$NA} & 68.7{\scriptsize $\pm$18.0} & 87.9{\scriptsize $\pm$6.1} & 88.8{\scriptsize $\pm$6.7} \\
0.4 & 51.3{\scriptsize $\pm$NA} & 50.8{\scriptsize $\pm$NA} & 49.8{\scriptsize $\pm$NA} & 70.7{\scriptsize $\pm$16.4} & 64.5{\scriptsize $\pm$6.9} & 66.6{\scriptsize $\pm$5.0} \\
0.6 & 50.7{\scriptsize $\pm$NA} & 49.7{\scriptsize $\pm$NA} & 49.5{\scriptsize $\pm$NA} & 65.3{\scriptsize $\pm$11.5} & 54.6{\scriptsize $\pm$4.4} & 55.1{\scriptsize $\pm$2.5} \\
0.8 & 50.5{\scriptsize $\pm$NA} & 49.9{\scriptsize $\pm$NA} & 49.7{\scriptsize $\pm$NA} & 57.7{\scriptsize $\pm$6.0} & 48.9{\scriptsize $\pm$1.7} & 49.2{\scriptsize $\pm$1.0} \\
\rowcolor{Gray} 1.0 & 50.0{\scriptsize $\pm$NA} & 49.8{\scriptsize $\pm$NA} & 50.0{\scriptsize $\pm$NA} & 50.0{\scriptsize $\pm$0.0} & 50.0{\scriptsize $\pm$0.0} & 50.0{\scriptsize $\pm$0.0} \\
1.2 & 50.3{\scriptsize $\pm$NA} & 48.5{\scriptsize $\pm$NA} & 50.8{\scriptsize $\pm$NA} & 48.7{\scriptsize $\pm$4.0} & 57.6{\scriptsize $\pm$1.8} & 57.8{\scriptsize $\pm$1.9} \\
1.4 & 54.5{\scriptsize $\pm$NA} & 46.7{\scriptsize $\pm$NA} & 55.8{\scriptsize $\pm$NA} & 50.8{\scriptsize $\pm$8.0} & 68.4{\scriptsize $\pm$3.4} & 68.4{\scriptsize $\pm$3.4} \\
1.6 & 58.6{\scriptsize $\pm$NA} & 44.5{\scriptsize $\pm$NA} & 63.5{\scriptsize $\pm$NA} & 55.4{\scriptsize $\pm$11.3} & 78.7{\scriptsize $\pm$3.6} & 78.6{\scriptsize $\pm$3.7} \\
1.8 & 64.9{\scriptsize $\pm$NA} & 41.6{\scriptsize $\pm$NA} & 71.6{\scriptsize $\pm$NA} & 62.1{\scriptsize $\pm$14.5} & 86.4{\scriptsize $\pm$3.5} & 86.3{\scriptsize $\pm$3.6} \\
2.0 & 75.8{\scriptsize $\pm$NA} & 38.4{\scriptsize $\pm$NA} & 79.3{\scriptsize $\pm$NA} & 67.3{\scriptsize $\pm$16.8} & 91.9{\scriptsize $\pm$3.0} & 91.7{\scriptsize $\pm$3.2} \\
2.5 & 95.6{\scriptsize $\pm$NA} & 31.1{\scriptsize $\pm$NA} & 89.8{\scriptsize $\pm$NA} & 76.2{\scriptsize $\pm$16.4} & 97.5{\scriptsize $\pm$1.5} & 97.4{\scriptsize $\pm$1.4} \\
3.0 & 98.4{\scriptsize $\pm$NA} & 25.8{\scriptsize $\pm$NA} & 90.7{\scriptsize $\pm$NA} & 82.8{\scriptsize $\pm$13.5} & 99.0{\scriptsize $\pm$0.6} & 99.0{\scriptsize $\pm$0.5} \\
3.5 & 99.3{\scriptsize $\pm$NA} & 21.7{\scriptsize $\pm$NA} & 93.7{\scriptsize $\pm$NA} & 88.1{\scriptsize $\pm$10.2} & 99.4{\scriptsize $\pm$0.3} & 99.4{\scriptsize $\pm$0.3} \\
4.0 & 99.8{\scriptsize $\pm$NA} & 18.0{\scriptsize $\pm$NA} & 96.4{\scriptsize $\pm$NA} & 90.7{\scriptsize $\pm$6.8} & 99.6{\scriptsize $\pm$0.3} & 99.6{\scriptsize $\pm$0.2} \\
4.5 &  100.0{\scriptsize $\pm$NA} & 14.9{\scriptsize $\pm$NA} & 97.4{\scriptsize $\pm$NA} & 91.7{\scriptsize $\pm$4.4} & 99.7{\scriptsize $\pm$0.2} & 99.7{\scriptsize $\pm$0.1} \\
5.0 &  100.0{\scriptsize $\pm$NA} & 11.7{\scriptsize $\pm$NA} & 98.1{\scriptsize $\pm$NA} & 91.7{\scriptsize $\pm$3.8} & 99.8{\scriptsize $\pm$0.1} & 99.7{\scriptsize $\pm$0.1} \\
5.5 &  100.0{\scriptsize $\pm$NA} & 9.7{\scriptsize $\pm$NA}& 98.5{\scriptsize $\pm$NA} & 91.0{\scriptsize $\pm$4.5} & 99.8{\scriptsize $\pm$0.1} & 99.8{\scriptsize $\pm$0.2} \\
6.0 &  100.0{\scriptsize $\pm$NA} & 7.9{\scriptsize $\pm$NA}& 98.7{\scriptsize $\pm$NA} & 89.7{\scriptsize $\pm$5.7} & 99.8{\scriptsize $\pm$0.1} & 99.8{\scriptsize $\pm$0.2} \\
6.5 &  100.0{\scriptsize $\pm$NA} & 7.0{\scriptsize $\pm$NA}& 98.9{\scriptsize $\pm$NA} & 88.3{\scriptsize $\pm$7.0} & 99.8{\scriptsize $\pm$0.2} & 99.8{\scriptsize $\pm$0.3} \\
\midrule
Average & 77.8 & 31.0 & 76.7 & 72.2 & \textbf{84.2} & \textbf{84.3} \\
 \bottomrule
 \end{tabular}}
\vspace{1.4mm}
\caption{NAS detection performance in regression task (age prediction) for NAS shift of brightness in RSNA boneage dataset measured by AUROC. Highlighted row presents the performance on the ID dataset. DE, MC Dropout, TAP-MB, and NA denotes Deep Ensemble, Monte Carlo Dropout, \emph{TAP-Mahalanobis}, and Not Applicable respectively. $\text{SWAG}^{*}$ = SWAG + Deep Ensemble. 
% Mahala and Mahala* indicate using penultimate layer only or ensembling all layer respectively.
}
\label{tab:regression_nas}
% \vspace{-1mm}

\end{table*}
% \end{wraptable}        

==> wacv/main_paper/tables/multi_class_nas_detection.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\footnotesize
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c c c  c  c  c c c  c c c}
\toprule
&\multicolumn{1}{c}{\multirow{1}{*}{Distribution}} & \multicolumn{1}{c}{\multirow{1}{*}{Brightness}} 
& \multicolumn{6}{c}{\multirow{1}{*}{Baselines}}  & \multicolumn{2}{c}{\multirow{1}{*}{Ours}} \\ \cmidrule(lr){4-9}  \cmidrule(lr){10-11} 
&\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{MSP~\cite{hendrycks2017base} } & \multicolumn{1}{c}{ODIN~\cite{liang2017enhancing} } & \multicolumn{1}{c}{Energy~\cite{liu2020energy} } & \multicolumn{1}{c}{MB~\cite{mahala18} } &  \multicolumn{1}{c}{KL~\cite{Hendrycks2019ABF} } &  \multicolumn{1}{c}{MOS~\cite{Huang2021MOSTS} } & \multicolumn{1}{c}{K = 32} & \multicolumn{1}{c}{K = 8}  

\\ \midrule
\parbox[t]{2mm}{\multirow{32}{*}{\rotatebox[origin=c]{90}{RSNA Bone Age}}}

 & \multirow{10}{*}{NAS} & 0.0 & 99.98 & 100.00 & 100.00 & 100.00 & 84.36 & 85.29 & 100.00 & 100.00 \\
 &  & 0.1 & 80.60 & 83.72 & 83.94 & 92.46 & 76.61 & 76.61 & 84.69 & 80.04 \\
 &  & 0.2 & 72.78 & 75.46 & 75.42 & 84.77 & 69.97 & 70.23 & 75.68 & 71.57 \\
 &  & 0.3 & 69.53 & 71.88 & 71.75 & 77.86 & 67.10 & 67.26 & 70.56 & 66.71 \\
 &  & 0.4 & 67.91 & 70.05 & 69.88 & 72.84 & 65.71 & 65.80 & 67.10 & 63.42 \\
 &  & 0.5 & 66.98 & 68.97 & 68.77 & 69.68 & 64.92 & 65.04 & 64.65 & 61.10 \\
 &  & 0.6 & 66.45 & 68.36 & 68.14 & 66.99 & 64.44 & 64.63 & 62.84 & 59.41 \\
 &  & 0.7 & 66.10 & 67.95 & 67.73 & 64.68 & 64.16 & 64.43 & 61.63 & 58.32 \\
 &  & 0.8 & 65.90 & 67.72 & 67.49 & 62.26 & 64.00 & 64.36 & 60.94 & 57.74 \\
 &  & 0.9 & 65.80 & 67.60 & 67.37 & 59.66 & 63.95 & 64.35 & 60.64 & 57.52 \\ \cdashline{2-11}[1pt/1pt]
 & ID & 1.0 & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 & 50.00 \\ \cdashline{2-11}[1pt/1pt]
 & \multirow{21}{*}{NAS} & 1.1 & 65.98 & 67.84 & 67.62 & 54.88 & 64.05 & 64.55 & 60.50 & 57.33 \\
 &  & 1.2 & 66.50 & 68.49 & 68.31 & 53.74 & 64.41 & 64.99 & 60.63 & 57.25 \\
 &  & 1.3 & 67.21 & 69.37 & 69.22 & 53.29 & 64.95 & 65.60 & 60.96 & 57.33 \\
 &  & 1.4 & 68.10 & 70.44 & 70.33 & 53.39 & 65.65 & 66.37 & 61.48 & 57.56 \\
 &  & 1.5 & 69.09 & 71.60 & 71.53 & 53.94 & 66.47 & 67.21 & 62.15 & 57.91 \\
 &  & 1.6 & 70.13 & 72.79 & 72.76 & 54.67 & 67.37 & 68.08 & 62.90 & 58.34 \\
 &  & 1.7 & 71.19 & 74.00 & 74.02 & 55.56 & 68.33 & 68.99 & 63.71 & 58.82 \\
 &  & 1.8 & 72.27 & 75.20 & 75.25 & 56.55 & 69.36 & 69.88 & 64.57 & 59.35 \\
 &  & 1.9 & 73.33 & 76.35 & 76.44 & 57.51 & 70.41 & 70.76 & 65.41 & 59.88 \\
 &  & 2.0 & 74.42 & 77.50 & 77.62 & 58.59 & 71.50 & 71.66 & 66.29 & 60.43 \\
 &  & 2.5 & 78.99 & 82.19 & 82.42 & 63.02 & 76.20 & 75.50 & 69.95 & 62.74 \\
 &  & 3.0 & 82.50 & 85.61 & 85.90 & 66.94 & 79.95 & 78.58 & 72.99 & 64.75 \\
 &  & 3.5 & 85.08 & 88.06 & 88.41 & 70.06 & 82.73 & 81.02 & 75.54 & 66.54 \\
 &  & 4.0 & 87.06 & 89.90 & 90.29 & 72.70 & 84.86 & 83.03 & 77.76 & 68.19 \\
 &  & 4.5 & 88.53 & 91.24 & 91.67 & 74.73 & 86.49 & 84.64 & 79.66 & 69.70 \\
 &  & 5.0 & 89.70 & 92.30 & 92.76 & 76.51 & 87.74 & 86.02 & 81.36 & 71.12 \\
 &  & 5.5 & 90.57 & 93.10 & 93.58 & 77.92 & 88.69 & 87.16 & 82.81 & 72.41 \\
 &  & 6.0 & 91.27 & 93.74 & 94.26 & 79.20 & 89.47 & 88.16 & 84.11 & 73.65 \\
 &  & 6.5 & 91.81 & 94.24 & 94.79 & 80.21 & 90.08 & 88.99 & 85.23 & 74.76 \\
 &  & 7.0 & 92.24 & 94.66 & 95.24 & 81.14 & 90.60 & 89.73 & 86.26 & 75.83 \\
 &  & 7.5 & 92.57 & 94.98 & 95.60 & 81.90 & 91.04 & 90.37 & 87.16 & 76.79 \\
 \bottomrule
\end{tabular}}
\caption{NAS detection performance for multi-class classification task on distributional shifts in RSNA boneage dataset measured by AUROC. \radhika{1. add plots for comparison in supplementary}
% Mahala and Mahala* indicate using penultimate layer only or ensembling all layer respectively.
}
\label{tab:binary_class_nas}
% \vspace{-4mm}
\end{table*}
